Data-Driven but Privacy-Conscious: Pedestrian Dataset De-identification via Full-Body Person Synthesis

The advent of data-driven technology solutions is accompanied by an increasing concern with data privacy. This is of particular importance for human-centered image recognition tasks, such as pedestrian detection, re-identification, and tracking. To highlight the importance of privacy issues and motivate future research, we motivate and introduce the Pedestrian Dataset De-Identification (PDI) task. PDI evaluates the degree of de-identification and downstream task training performance for a given de-identification method. As a first baseline, we propose IncogniMOT, a two-stage full-body de-identification pipeline based on image synthesis via generative adversarial networks. The first stage replaces target pedestrians with synthetic identities. To improve downstream task performance, we then apply stage two, which blends and adapts the synthetic image parts into the data. To demonstrate the effectiveness of IncogniMOT, we generate a fully de-identified version of the MOT17 pedestrian tracking dataset and analyze its application as training data for pedestrian re-identification, detection, and tracking models. Furthermore, we show how our data is able to narrow the synthetic-to-real performance gap in a privacy-conscious manner.

==> figures/qualitative_pose2person.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=0.65\textwidth, trim={0px 0px 210px 0px}, clip]{figures/supp_qualitat2.pdf}
\end{center}
   \caption{
   %
   \textbf{Qualitative results} and input poses of our AnonyMOT anonymization method.
   %
   In the first row we show the original images from different times identities and sequences.
   %
   The second row shows their respective pose information used as an input to \netone.
   %
   The third row shows the blending and adaption with our \nettwo into the given scene.
   }
\label{fig:qualitative_pose2person}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sections_censor/preamble.tex <==
\usepackage{graphicx}
% DO NOT USE \usepackage{times}, it will be removed by typesetters
%\usepackage{times}

\usepackage{tikz}
\usepackage{comment}
\usepackage{amsmath} % define this before the line numbering.
\usepackage{amssymb}
\usepackage{color}


\usepackage{booktabs}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{array}
\usepackage{soul}
\usepackage{enumitem}

\usepackage{floatrow}
\usepackage{subfig}
\usepackage{xspace}

\usepackage{caption}
% \usepackage{subcaption}
% \usepackage{subfigure}
\usepackage{wrapfig}

\usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
\newfloatcommand{capbtabbox}{table}[][\FBwidth]

\usepackage{blindtext}

%\usepackage[capitalize]{cleveref} 

% The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.

% INITIAL SUBMISSION - The following two lines are NOT commented
% CAMERA READY - Comment OUT the following two lines
\usepackage{ruler}
\usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}

\definecolor{citecolor}{RGB}{34,139,34}
\usepackage[pagebackref=true,breaklinks=true,colorlinks,citecolor=citecolor,bookmarks=false]{hyperref}
\usepackage{cite}

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
% introduce hidden column type
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}

\usepackage[capitalize]{cleveref} 
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

\newcommand{\netone}{{\emph{Pose2PersonNet}}\@\xspace}
\newcommand{\nettwo}{{\emph{Person2SceneNet}}\@\xspace}
\newcommand{\stageone}{{\emph{Pose2Person}}\@\xspace}
\newcommand{\stagetwo}{{\emph{Person2Scene}}\@\xspace}

\newcommand{\tim}[1]{\textcolor{blue}{TIM: #1}}
\newcommand{\mm}[1]{\textcolor{teal}{MAXIM: #1}}
\newcommand{\ili}[1]{\textcolor{orange}{ISMAIL: #1}}
\newcommand{\lau}[1]{\textcolor{magenta}{LAURA: #1}}
\newcommand{\alj}[1]{\textcolor{violet}{ALJOSA: #1}}

\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}


\newcommand{\crefrangeconjunction}{--}
